Group Distributionally Robust Dataset Distillation with Risk Minimization

Dataset distillation (DD) has emerged as a widely adopted technique for crafting a synthetic dataset that captures the essential information of a training dataset, facilitating the training of accurate neural models. Its applications span various domains, including transfer learning, federated learning, and neural architecture search. The most popular methods for constructing the synthetic data rely on matching the convergence properties of training the model with the synthetic dataset and the training dataset. However, using the empirical loss as the criterion must be thought of as auxiliary in the same sense that the training set is an approximate substitute for the population distribution, and the latter is the data of interest. Yet despite its popularity, an aspect that remains unexplored is the relationship of DD to its generalization, particularly across uncommon subgroups. That is, how can we ensure that a model trained on the synthetic dataset performs well when faced with samples from regions with low population density? Here, the representativeness and coverage of the dataset become salient over the guaranteed training error at inference. Drawing inspiration from distributionally robust optimization, we introduce an algorithm that combines clustering with the minimization of a risk measure on the loss to conduct DD. We provide a theoretical rationale for our approach and demonstrate its effective generalization and robustness across subgroups through numerical experiments. The source code is available at https://github.com/Mming11/RobustDatasetDistillation.

==> Tables/ablation.tex <==
\begin{table}[t]

\caption{\label{tab:ablation}Ablation study on CVaR loss. The experiment is conducted on CIFAR-10 and ImageNet-A under 10 IPC. The baseline model is GLaD. ``CE'' denotes cross entropy loss, and ``CL'' refers to cluster accuracy. The best results are marked in \textbf{bold}. }
\centering
\small
\begin{tabular}{cccccccc}
\toprule
    \multicolumn{3}{c}{Loss} & \multicolumn{2}{c}{CIFAR-10} & \multicolumn{2}{c}{ImageNet-A} \\
    \multirow{2}{*}{CE} & CVaR & CVaR & \multirow{2}{*}{Acc} & CL & \multirow{2}{*}{Acc} & CL \\
    & -avg & -max & & -min & & -min \\
\midrule
    \checkmark & - & - & 46.7 & 40.2 & 53.9 & 40.5 \\
    \checkmark & \checkmark & - & 49.1 & 45.3 & 56.4 & 43.9 \\
    \checkmark & - & \checkmark & 47.9 & 44.2 & 56.1 & 43.7 \\
    \checkmark & \checkmark & \checkmark & \textbf{50.2} & \textbf{46.7} & \textbf{57.5} & \textbf{45.8} \\
\bottomrule
\end{tabular}
\end{table}

==> Tables/efficiency-evaluation.tex <==
\begin{table}[t]
\caption{\label{tab:efficiency-evaluation}Efficiency evaluation over the CIFAR dataset in comparision with the baseline method. The experiment is conducted on CIFAR-10 under 10 IPC settings. The baseline method is IDC. }
\centering
\small
\begin{tabular}{ccc}
\toprule
    & IDC & IDC$^\mathcal{R}$ \\
\midrule
    Time & 70s & 100s \\
\bottomrule
\end{tabular}
\end{table}
